Dynamic Data Structures for Interval Coloring

We consider the dynamic graph coloring problem restricted to the class of interval graphs. At each update step the algorithm is presented with an interval to be colored, or a previously colored interval to delete. The goal of the algorithm is to efficiently maintain a proper coloring of the intervals with as few colors as possible by an online algorithm. In the incremental model, each update step presents the algorithm with an interval to be colored. The problem is closely connected to the online vertex coloring problem of interval graphs for which the Kierstead-Trotter (KT) algorithm achieves the best possible competitive ratio. We first show that a sub-quadratic time direct implementation of the KT-algorithm is unlikely to exist conditioned on the correctness of the Online Boolean Matrix Vector multiplication conjecture due to Henzinger et al. \cite{DBLP:conf/stoc/HenzingerKNS15}. We then design an incremental algorithm that is subtly different from the KT-algorithm and uses at most $3 \omega - 2$ colors, where $\omega$ is the maximum clique in the interval graph associated with the set of intervals. Our incremental data structure maintains a proper coloring in amortized $O(\log n + \Delta)$ update time where $n$ is the total number of intervals inserted and $\Delta$ is the maximum degree of a vertex in the interval graph. We then consider the fully dynamic framework involving insertions and deletions. On each update, our aim is to maintain a $3 \omega - 2$ coloring of the remaining set of intervals, where $\omega$ is the maximum clique in the interval graph associated with the remaining set of intervals. Our fully dynamic algorithm supports insertion of an interval in $O(\log n + \Delta \log \omega)$ worst case update time and deletion of an interval in $O(\Delta^2 \log n)$ worst case update time.

==> Journal/FullyDynamic_copy.tex <==
\section{Fully dynamic interval coloring}
\label{sec:fully-dynamic-algorithm}
In this section we consider interval coloring in the fully dynamic setting. The update sequence allows  update for insertion of a new interval and deletion of a previously colored interval. In the fully dynamic setting, $I_i$ represents the interval inserted in the $i$-th update step and value of $i$ ranges from $1$ to {\sf U}, where {\sf U} is the total number of updates. In the update sequence, an update of type {\sf Insert$(I_i)$} signifies that the current update is the $i$-th update which is presenting a new interval to the algorithm for insertion. An update of type {\sf Delete$(I_i)$} signifies that the interval $I_i$ with color $(L(I_i), o(I_i))$, which was inserted previously in the $i$-th update, is presented to the algorithm for deletion.\par
We use $\Insertion$ (Algorithm~\ref{alg:insert}) for insertion of a new interval, but with a different set of data structures to maintain SLS (see Section~\ref{subsec:DSpreliminaries}). To handle deletion of an interval $I_i$, we use algorithm $\Deletion$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Algorithm $\Deletion$}
\label{subsec:deletionAlgo} 
Let $I_i = [l_i,r_i]$ with color $(L(I_i),o(I_i))$ be the interval presented for deletion in the current update step. We present pseudo code of $\Deletion$ in Algorithm~\ref{alg:delete}.
%and a summarized description of the procedures used in Algorithm~\ref{alg:delete} in Table~\ref{table:3}. 
Algorithm $\Deletion$ supports deletion of an interval by implementing the steps as described below:\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\bf Step 1:} Remove interval $I_i$ from the set of intervals $\mathcal{I}$ and hash table $T[L(I_i)]$.(Line 1 and Line 2 in Algorithm~\ref{alg:delete})\\
{\bf Step 2:} Compute the set of endpoints contained in $I_i$. Let $\mathcal{E}_i$ = $\mathcal{E} \cap I_i$. (Line 3 in Algorithm~\ref{alg:delete})\\
\textbf{Step 3:} For each endpoint $t \in \mathcal{E}_i$, update SLS $e_t$  to reflect the deletion of interval $I_i$. (Line 4 to 8 in Algorithm~\ref{alg:delete})\\
\textbf{Step 4:} Compute the set of intervals intersecting with $I_i$ and with level value strictly greater than $L(I_i)$. Let 
$\D$ = $\{I_j | L(I_j) > L(I_i), I_i \cap I_j \neq \phi\}$ (Line 9 in Algorithm~\ref{alg:delete}). Sort $\D$ in the increasing order of level value and break the ties in the increasing order of time of insertion.
For every interval $I_j$ in $\D$, repeat the following steps:
\begin{itemize}
	\item Compute the set of endpoints intersecting with $I_j$. Let $S$ = $\mathcal{E} \cap I_j$. For every endpoint $t \in S$ compute the height $h_t$ of the SLS $e_t$. Compute $h$ = $\max\{h_t | t \in S\}$ (Line 11 in Algorithm~\ref{alg:delete}).
	\item If $h \geq L(I_j)$ then no further processing is required for interval $I_j$. 
	%Then $L(I_j)$ is unchanged. Prior to this update, we maintained invariant $\C$ for interval $I_j$. Invariant $\C$ persists for $I_j$ after the update.
	\item If $h < L(I_j)$ then following steps are executed (Line 17 to 25 in Algorithm~\ref{alg:delete}):
	%, Invariant $\C$ is violated for $I_j$. Following steps are executed to restore Invariant $\C$ for $I_j$ (Line 17 to 25 in Algorithm~\ref{alg:delete}):
	\begin{itemize}
		\item Change level value of $I_j$ from $L(I_j)$ to $h$.  %This ensures that  there is a $t \in I_j$ such that $h_t \geq L(I_j)+1$.  Therefore, invariant $\C$ is restored for $I_j$. 
		\item Recompute the offset value $o(I_j)$ for $I_j$ with the new level value $h$.
		\item Update SLS $e_t$ for every point $t \in S$ to reflect the change in level value of $I_j$. 
	\end{itemize}
\end{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[H]	
	\caption{$\Deletion$($I_i = [l_i,r_i]$) is used to handle deletion of interval $I_i$}
	\begin{algorithmic}[1]
		\State $T[L(I_i)].$delete$(I_{i})$
		\State $\mathcal{I}$.delete($I_{i}$)
		\State $\mathcal{E}_i \leftarrow \mathcal{E}$.intersection($I_{i}$)
		\For{$t$ \textbf{in} $\mathcal{E}_i$}
		\If{$\mid T[L(I_i)]$.intersection($t) \mid$ $ = 0$}
		\State ${NZ}_t$.delete($L(I_i)$ $\And$ $Z_t$.insert($L(I_i)$)
		%\State $Z_t$.insert($L(I_i)$)
		\EndIf
		\EndFor
		\State{Compute $\D \leftarrow \{I_j | L(I_j) > L(I_i), I_i \cap I_j \neq \phi\}$. Sort $\D$ in the increasing order of level value and break the ties in the increasing order of time of insertion.} 
		\For{$I_j$ \textbf{in} $\D$}
		\State $S, h \leftarrow $ \Call{$\computemaxheightSLS$}{$\mathcal{E}$,$I_j$}
		\If{$h \geq L(I_j)$} 
		\State \textbf{continue}
		\EndIf
		\State $T[L(I_j)].$delete($I_j$)
		\State $T[h].$insert($I_j$)
		\For{$t$ \textbf{in} $S$}
		\If{$\mid T[L(I_j)]$.intersection($t) \mid$ $= 0$}
		\State ${NZ}_t$.delete($L(I_j)$ $\And$ $Z_t$.insert($L(I_j)$)
		\EndIf
		\State {${NZ}_t$.insert($h$) $\And$ $Z_t$.delete($h$)}
		\EndFor
		\State $L(I_j) \leftarrow h$
		\State \Call{$\OFFSET$}{$I_j$}
		\EndFor
		
	\end{algorithmic}
	\label{alg:delete}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Correctness of $\Deletion$}
\label{subsec:correctnessDeletionAlgo}
In the case of  deletion of an interval, it is crucial to ensure that level value assigned to any new interval after a deletion is at most $\omega - 1$ and such an interval satisfies property {\bf P}. In order to achieve the same, every interval $I_j$ which remains after a deletion must satisfy the following invariant:\\    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\bf Invariant $\C$:} An interval $I_j$ is said to satisfy Invariant $\C$ if there exists an endpoint $t$ contained in $I_j$ such that the height of the SLS at $t$ is at least $L(I_j)$.\par 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%An interval is called \textit{dirty} after a deletion if invariant $\C$ is violated for that interval. An interval which is not dirty after a deletion is called \textit{clean}.
%Let $\D$ denotes the set of all dirty intervals after the deletion of interval $I_i$.
Lemma~\ref{lem:3-competitive-fully-dynamic} shows that maintaining invariant $\C$ ensures property {\bf P}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
	\label{lem:3-competitive-fully-dynamic}
	At the end of each update, the number of colors used is  at most $3 \omega - 2$, where $\omega$ is the size of the maximum clique in the interval graph just after the update.	
\end{lemma}
\begin{proof}
If the update is inserting an interval then it is easy to observe that the algorithm maintains invariant $\C$. This is because, prior to the insertion, invariant $\C$ was satisfied by all the intervals. After the insertion, because of the way level value and offset value are computed by $\Insertion$, the newly inserted interval also satisfies invariant $\C$.
If the update deletes an interval $I_i$ then the only set of intervals which may get affected is the set of intervals intersecting with $I_i$ and with level value strictly greater than $L(I_i)$ (Lemma~\ref{lem:set-of-dirty-intervals}). Algorithm $\Deletion$ includes all such intervals in the set $\D$ and ensures that for each interval $I_j \in \D$, there is a point $t \in I_j$ such that
$h_t \geq L(I_j)$. Further,  for each $I_j \in \D$  the algorithm maintains the following invariant that  whenever $L(I_j)$ is modified: 
$L(I_j)$ is modified to be the maximum $h_t$, over all $t \in I_j$. Therefore, algorithms $\Insertion$ and $\Deletion$ maintains invariant $\C$.\par %that after every update, for each interval $I_i$, there is a point $t \in I_i$ such that $h_t \geq L(I_i)$.\par  
The same arguments in Lemma~\ref{lem: Property-P} proves that $\Insertion$ satisfies Property {\bf P}. For $\Deletion$, invariant $\C$ ensures the largest level value of any interval is at most $\omega - 1$.  Further, the intervals whose level values are $0$ form an independent set.     
	%Further,  for each $I_j \in \D$  the algorithm maintains the following invariant that  whenever $L(I_j)$ is modified: 
	%$L(I_j)$ is modified to be the maximum $h_t$, over all $t \in I_j$.  
Next, we claim that in $\Deletion$ when $L(I_j)$ changes it has at most two neighbors in the new level and none of the neighbors has a containment relationship with $I_j$.  The proof is by contradiction by assuming that $I_j$ is the first interval for which this claim is false.  The contradiction is obtained by using the argument in Lemma~\ref{lem: Property-P}.\par 
Therefore, it follows that after the update step, Property ${\bf P}$ is satisfied by the level assignment to the intervals.  Consequently, the algorithm uses at most $3 \omega - 2 $ colors after each update step. Hence the Lemma.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
An interval is called \textit{dirty} after a deletion if invariant $\C$ is violated for that interval. An interval which is not dirty after a deletion is called \textit{clean}.
In Lemma~\ref{lem:set-of-dirty-intervals}, we show that $\D$ is a super set of all such intervals which may become dirty after a delete. 
The efficiency of the deletion update depends on the efficient computation of the set $\D$ and clean-up of $\D$ so that at the end of the update, there are no dirty intervals.  We also must ensure that during the clean-up of the set $\D$ no clean interval becomes dirty. On deletion of interval $I_i$, we initialize the set $\D$ = $\{I_j | L(I_j) > L(I_i), I_i \cap I_j \neq \phi\}$. In other words, the set $\D$ consists of every interval $I_j$ such that $L(I_j) > L(I_i)$ and $I_j$ intersects with $I_i$. Then, $\D$ is sorted in the increasing order of level value of the intervals and ties are broken in the increasing order of time of insertion.  
%Lemma \ref{lem:set-of-dirty-intervals} shows that set $\D$ is a superset of all intervals which became dirty after deletion of interval $I_i$.  Thus we bound the set $\D$ by showing that only those intervals which are adjacent to $I_i$ and whose level value is more than $L(I_i)$ can be dirty during the deletion of $I_i$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
	\label{lem:set-of-dirty-intervals}
	Let $I_i$ be the deleted interval and let $(L(I_i),o(I_i))$ be the color of  $I_i$. Then the set $\D$ is a super set of all the intervals those may become dirty after the delete. 
\end{lemma} 
\begin{proof}
%	Let $I_k$ be an interval.  By the definition of level value of an interval, we know that there is a point $t \in I_k$ such that $h_t \geq L(I_k)$.  In other words, for  the SLS $e_t = \{(t,0), \ldots, (t,h_t-1)\}$, $h_t$ is at least $L(I_k)$.  Further, $\Deletion$  maintains invariant $\C$ and thus ensures that, for every interval $I_j$ intersecting with $I_i$, whenever $L(I_j)$ is modified it is changed to be the maximum $h_t$, over all $t \in I_j$. Also, the intervals are processed in non-decreasing order of level number, and the level number is not increased.\\
After deletion of $I_i$, if for any endpoint $t \in I_i$ the height of SLS $e_t$ changes then it only decreases and the changed height is at least $L(I_i)$. The claim is immediate from the definition of height of an SLS in Definition~\ref{def:SLS}.\\ 
%Further, since $\Deletion$ process the set $\D$ in the increasing order of level value, the changed height for the SLS also shows an increasing order starting from $L(I_i)$.\\ 
Firstly, we show that for an interval $I_k$, if  $L(I_k) \leq L(I_i)$ then $I_k$ does not become dirty due to the deletion of $I_i$ and during the update. This is because, for any SLS $e_t$ contained in $I_k$ if the height $h_t$ changes due to deletion of interval $I_i$ then the new value of $h_t$ is at least $L(I_i)$. 
Since $L(I_i) \geq L(I_k)$, we have $h_t \geq L(I_k)$ and hence SLS $e_t$ maintains invariant $\C$ for interval $I_k$. Further, since intervals in set $\D$ has level value strictly more than $L(I_i)$, $h_t$  remains at least $L(I_k)$ during processing of set $\D$.\\
Secondly, we show that if $I_k \cap I_i = \phi$, then $I_k$ does not become dirty due to the deletion of $I_i$ and during the  update.  If $I_k \cap I_i = \phi$, then the intervals $I_k$ and $I_i$ are disjoint. Therefore, if an endpoint $t \in I_k$ then $h_t$ does not change due to deletion of $I_i$. To complete the claim, we further need to show that during processing the set $\D$, $I_k$ does not become dirty. Suppose not and let $I_j$ be the first interval in $\D$ such that $I_k$ becomes dirty after a decrease in $L(I_j)$. This implies that $L(I_k) > L(I_j) > L(I_i)$. Further, for any endpoint $t \in I_k$, $h_t < L(I_k)$, after a decrease in $L(I_j)$ . 
Since $I_k$ was clean prior to processing $I_j$, there must exists an endpoint $t^{\prime}$, such that $t^{\prime} \in I_j \cap I_k$ and prior to decrease in  $L(I_j)$ the following holds: $h_t^{\prime} \geq L(I_k) > L(I_j)$. 
But then from the definition of height of SLS, there must be an interval at every level $x$, $0 \leq x < L(I_k)$. Since $L(I_k) > L(I_j)$, at the time of processing $I_j$, there exist an interval containing endpoint $t^{\prime}$ at every level $x$, $0 \leq x < L(I_j)$. This contradicts that $L(I_j)$ is decreased at the time of processing $I_j$. Therefore, such an interval $I_j$ does not exist. Hence the Lemma.     
%Therefore, $t \not\in I_i$.  Consequently,  it follows that for each $0 \leq x \leq h_t-1$  during the update the level is unchanged for the  interval $I_p$ for which $t \in I_p$ and $L(v_p) = x$.  Therefore, the maximum height of supporting line segments in $I_k$ after the deletion of $I_i$ and throughout the update is at least $h_t$.  Since $h_t \geq L(I_k)$ after the deletion of $I_i$ it follows that $I_k \not \in \D$. Hence the lemma.\\
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Procedures used in $\Deletion$ and $\Insertion$}
\label{subsec:procedureHandleDeleteInsert}
We use the same procedures as described in Section~\ref{subssec:procedures-handle-insert} in $\Deletion$ and $\Insertion$. But in the fully dynamic setting, SLS is maintained using Red-Black trees and hence running time of the procedures differ from those described in Section~\ref{subssec:procedures-handle-insert}. For the purpose of completeness we describe the procedures again along with running time analysis. A summarized description of the procedures is given in Table~\ref{table:3}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{enumerate}
\item \textbf{Procedure $\getSLS$$(\mathcal{I},t)$: }This procedure is used to compute the SLS at endpoint $t$. It works as follows (Algorithm~\ref{alg:GET-SLS}):  
an intersection query is performed on $\mathcal{I}$ with $[t,t]$. The query returns all the intervals in $\mathcal{I}$ which contain endpoint $t$. Let $\mathcal{I}_{t}$ denote the set returned by the intersection query. Red-Black trees $Z_{t}$ and ${NZ}_{t}$, each of size $\max(levels(\mathcal{I}_{t}))$, are created. For every $i$ in the range $[0,\max(levels(\mathcal{I}_{t}))]$, 
if $i \in levels(\mathcal{I}_{t})$ then $i$ is inserted to $Z_{t}$. Otherwise, $i$ is inserted to ${NZ}_{t}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[H]
	\caption{$\getSLS$($\mathcal{I}$,$t$) is used to compute the supporting line segment at endpoint $t$. In this procedure SLS is maintained using Red-Black Trees.}
	\begin{algorithmic}[1]
		\Procedure{$\getSLS$}{$\mathcal{I}$,$t$}
		\State $\mathcal{I}_t \leftarrow$  $\mathcal{I}$.intersection($[t,t]$)
		\State $h_t \leftarrow 0$
		\State{$U \leftarrow$ Initialize to empty set}
		\For{$I$ \textbf{in} $\mathcal{I}_t$}
		\State ${U}.$insert($L(I)$)
		\State $h_t \leftarrow max(h_t,L(I))$
		\EndFor
		\State $Z_t \leftarrow $ Empty Red-Black tree
		\State $NZ_t \leftarrow $ Empty Red-Black tree
		\For{$i$ \textbf{in} $\{0,1,2,...h_t\}$} 
		\State $Z_t.$insert($i$)
		\EndFor
		\For{$i$ \textbf{in} $U$.begin() \textbf{to} $U$.end()} 
		\State ${NZ}_t.$insert($i$)
		\State $Z_t.$delete($i$)
		\EndFor
		\State \Return $Z_t, {NZ}_t$
		\EndProcedure
	\end{algorithmic}
	\label{alg:GET-SLS}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{lem:runtimeComputeSLSfullyDynamic}	
Procedure $\getSLS$ takes $O(\log n + \omega \log \omega)$ time.
\end{lemma}
\begin{proof}
Intersection query takes $O(\log|\mathcal{I}| + |\mathcal{I}_t|)$ time. At any level, SLS ${e_t}$ intersects with at most $2$ intervals and we have $\omega$ many levels. Hence, $|\mathcal{I}_{t}|$ = $O(\omega)$. Again, $|\mathcal{I}| \leq n$.	Therefore, $O(\log|\mathcal{I}| + |\mathcal{I}_t|)$ = $O(\log n + \omega)$. 
For the SLS $e_t$, at most $\omega$ insertions are required in the Red-Black tree $Z_{t}$ and ${NZ}_{t}$. A single insertion in $Z_{t}$ and ${NZ}_{t}$ takes $O(\log \omega)$ time. Therefore, total time taken for all the operations on $Z_{t}$ and ${NZ}_{t}$ is $O(\omega \log \omega)$. Therefore, worst case time taken by $\getSLS$ is $O(\log n + \omega \log \omega)$. Hence the Lemma.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item \textbf{Procedure $\computemaxheightSLS$$(\mathcal{E},I)$: }This procedure is used to compute the maximum height of SLS contained in interval $I_i$. It works as follows (Algorithm~\ref{alg:MAX-HEIGHT-OF-SLS-IN-INTRVAL}): an intersection query is performed on $\mathcal{E}$ with $I_i$. Let $S$ be the set returned by the intersection query.
For every endpoint $t \in S$, to compute the height $h_t$ of SLS $e_t$, the following steps are used: If $Z_t$ is non empty then the minimum value in $Z_t$ is assigned to $h_t$. Otherwise, $h_t$ is assigned a value which is one more than the maximum value in ${NZ}_t$. The maximum value of the height of an SLS at any endpoint in $S$ is computed as $h$ = $\max \{h_t | t \in S\}$. The procedure returns the set $S$ and value $h$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[H]
	\caption{$\computemaxheightSLS$($\mathcal{E}$,$I$) is used to compute the set $S$ of endpoints contained in interval $I$ and compute the maximum height $h$ of all the supporting line segments at these endpoints. In this procedure SLS is maintained using Red-Black Trees.}
	\begin{algorithmic}[1]
		\Procedure{$\computemaxheightSLS$}{$\mathcal{E}$,$I$} 
		\State $S \leftarrow$  $\mathcal{E}$.intersection($I$)
		\State $h \leftarrow 0$
		\For{$t$ \textbf{in} $S$}
		\If{$Z_t$.empty() $\And$ ${NZ}_t$.empty()}
		\State $h_t \leftarrow $ 0
		\ElsIf{$Z_t$.empty()}
		\State $h_t \leftarrow {{NZ}_t}.\max()+1$
		\Else 
		\State $h_t \leftarrow {Z_t}.\min()$
		\EndIf
		\State $h \leftarrow \max(h,h_t)$
		\EndFor
		\State return $S, h$
		\EndProcedure
	\end{algorithmic}
	\label{alg:MAX-HEIGHT-OF-SLS-IN-INTRVAL}
\end{algorithm}	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{lem:runtimeComputemaxheightfullydynamic}	
Procedure $\computemaxheightSLS$ takes $O(\log n + \Delta \log \omega)$ time.
\end{lemma}
\begin{proof}
We know that $|S| \leq \Delta$ and $|\mathcal{E}| \leq 2n$.	
Therefore, time taken to obtain the set $S$ is $O(\log n + \Delta)$. For every endpoint $t \in S$, the height $h_t$ of SLS $e_t$ is obtained in $O(\log \omega)$ time.   
Therefore, to obtain the height of supporting line segments at all the points in $S$, total time required is $O(\Delta \log \omega)$. Finding the maximum height takes another $O(\Delta)$ time. Therefore, worst case time taken by $\computemaxheightSLS$ is $O(\log n + \Delta \log \omega)$. Hence the Lemma.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item \textbf{Procedure $\updateEndPoints$$(S, L(I))$: }This procedure is used to update the SLS at the endpoints contained in set $S$. It works as follows (Algorithm~\ref{algo:UPDATE-EDGE-POINTS}): for every $ t \in S$, $L(I_i)$ is deleted from $Z_t$ and inserted to ${NZ}_t$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[H]
	\caption{$\updateEndPoints$($S,L(I)$) is used to update the supporting line segments at the endpoints contained in set $S$ for level value $L(I)$. In this procedure SLS is maintained using Red-Black Trees.}
	\begin{algorithmic}[1]
		\Procedure{$\updateEndPoints$}{$S$,$L(I)$} 
		\For{$t$ \textbf{in} $S$}
		\If{$ \neg Z_t$.empty()}
		\State{$h_t \leftarrow {Z_t}.min()$}
		\EndIf
		\If{$Z_t$.empty()}
		\State{$h_t \leftarrow {{NZ}_t}.max() + 1$}
		\EndIf
		\State{$q$ = $h_t$}    
		\While{$q < L(I)$} 
		\State ${Z_t}.$insert$(q)$
		\State{ $q \leftarrow q + 1$} 
		\EndWhile
		\If{$L(I)$ \textbf{in} $Z_t$} 
		\State ${Z_t}.$delete$(L(I))$ 
		\EndIf
		\State ${{NZ}_t}.$insert$(L(I))$
		\EndFor
		\EndProcedure
	\end{algorithmic}
	\label{algo:UPDATE-EDGE-POINTS}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{lem:runtimeUpdaeSLSfullydynamic}	
Procedure $\updateEndPoints$ takes $O(\Delta \log \omega)$ time.
\end{lemma}
\begin{proof}
The procedure works as follows: 
for every $ t \in S$, $L(I_i)$ is deleted from $Z_t$ and $L(I_i)$ inserted to ${NZ}_t$. For one SLS $e_t$ it takes $O(\log \omega)$ time and $|S| \leq \Delta$. Therefore, worst case time taken by $\updateEndPoints$ is $O(\Delta \log \omega)$. Hence the Lemma.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\item \textbf{Procedure $\OFFSET$$(I_i)$:} This procedure is same as the one described in Section~\ref{subssec:procedures-handle-insert}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
	\centering 
	\begin{tabular}{|l|l|l|} 
		\hline
		\multicolumn{3}{|l|}{$\getSLS$$(\mathcal{I},t)$}\\
		\hline
		Description & Worst-case  & Return\\
		& Running Time & Value \\
		\hline
		Computes the supporting line segment for endpoint $t$ & $O(\log(n)+\omega \log \omega)$ & $Z_t, {NZ}_t$\\
		and maintains it as the Red Black Tree $Z_t$ and ${NZ}_t$.  & (Lemma~\ref{lem:runtimeComputeSLSfullyDynamic}) & \\
		\hline
		\hline
		\multicolumn{3}{|l|}{$\computemaxheightSLS$$(\mathcal{E},I_i)$}\\
		\hline
		Description & Worst-case  & Return\\
		& Running Time & Value \\
		\hline
		From the interval tree $\mathcal{E}$, computes the set of endpoints $S$   & $O(\log(n)+\Delta \log \omega)$ & $S,h$\\
		contained in the interval $I_i$ and for each $t \in S$, & & \\
		using the Red Black trees $Z_t$ and ${NZ}_t$,  computes the  height $h_t$  & (Lemma~\ref{lem:runtimeComputemaxheightfullydynamic}) & \\
		and returns the maximum height $h$ = $\max\{h_t | t \in S \}$ & & \\
		\hline
		\hline
		\multicolumn{3}{|l|}{$\updateEndPoints$$(S,L(I_i))$}\\
		\hline
		Description & Worst-case & Return \\
		& Running Time & Value \\
		\hline
		Updates the endpoints in $S$ . & $O(\Delta \log \omega)$ & - \\
		to reflect the addition of a new interval $I_i$ at level $L(I_i)$.  & (Lemma~\ref{lem:runtimeUpdaeSLSfullydynamic}) & \\
		This updates the  Red Blach trees $Z_t$ and ${NZ}_t$ for each $t \in S$ & & \\
		\hline
		\hline
		\multicolumn{3}{|l|}{$\OFFSET$$(I)$}\\
		\hline
		Description & Worst-case & Return\\
		& Running Time & Value \\
		\hline
		Assigns an offset value to $v$ from $\{1,2,3\}$ & $O(\log(n))$ & -\\
		by considering the offset of the intervals  & (Lemma~\ref{lem:time-greeyd-coloring}) & \\
		intersecting it in $T[L(I)]$ where $L(I)$ is the level value of $I$ & & \\
		\hline
	\end{tabular}
	\caption{Procedures used in $\Insertion$ and $\Deletion$}
	\label{table:3}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
In this section we describe the different procedures used in our fully dynamic algorithm. %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
To address the issues mentioned in challenge 1, Algorithm~\ref{alg:delete} does the following after deletion of an interval $I_i$: Interval $I_i$ is deleted from interval tree $I$ and $T[L(I_i)]$. To find the set of endpoints $E_{I_i}$, a query is performed on the interval tree $\mathcal{E}$ with interval $I_i$. For every endpoint $t \in E_{I_i}$, a query is performed on $T[L(I_i)]$. If this query returns NULL then $L(I_i)$ is deleted from the Red-Black tree $NZ_{t}$ and $L(I_i)$ is inserted to the Red-Black tree $Z_t$.\par 
%We analyze all these operations in details in Section~\ref{subsec:analysis-fully-dynamic-algorithm}.\par 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We present a description of the use of different data structures and procedures in realizing the steps of Algorithm~\ref{alg:delete} and $\Insertion$ (Algorithm~\ref{alg:insert}) in the fully dynamic setting. We give a summarized description of the procedures in Table~\ref{table:3}. 
\begin{description}
\item[\textbf{Data structures and procedures used in $\Deletion$:}] Let $I_i = [l_i,r_i]$ with color $(L(I_i), o(I_i))$ be the interval presented to Algorithm~\ref{alg:delete} for deletion. Algorithm~\ref{alg:delete} involves $4$ steps.\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Step 1:} Interval $I_i$ is removed from interval tree $\mathcal{I}$ and interval tree $T[L(I_i)]$.\\
\textbf{Step 2:} To compute $E_{I_i}$ = $\mathcal{E} \cap I_i$, an intersection query is performed on $\mathcal{E}$ with $I_i$.\\  
\textbf{Step 3:} For every endpoint $t \in E_{I_i}$, SLS $e_t$ needs to be updated. To do so, it is required to check if there is another interval with level value equal to $L(I_i)$ that contains $t$. From property \textbf{P}, after deletion of $I_i$, there can be at most two intervals with level value $L(I_i)$ that contains $t$. To complete this check, an intersection query is performed on $T[L(I_i)]$ with $t$. If the query returns a NULL, then $L(I_i)$ is deleted from the tree ${NZ}_t$ and $L(I_i)$ is inserted into the tree $Z_t$.\\
\textbf{Step 4:} Set $\D$ = $\{I_j | L(I_j) > L(I_i), I_i\cap I_j \neq \phi\}$ needs to be computed. To compute $\D$, an intersection query is performed on $\mathcal{I}$ with $I_i$. Let $H$ be the set returned by this query. Clearly $\D \subseteq H$. The set $H$ is searched linearly and any interval with level value at most $L(I_i)$ is discarded. The remaining intervals are sorted in the increasing order of their level value and ties are broken in the increasing order of insertion time. Finally, the sorted set of the remaining intervals is the required set $\D$. Every interval $I_j$ in the set $\D$ is processed as follows:
\begin{itemize}
	\item To compute the set $S$ of supporting line segments contained in $I_j$ and the maximum height of any SLS in $S$ procedure $\computemaxheightSLS$$(\mathcal{E}, I_j)$ (Algorithm~\ref{alg:MAX-HEIGHT-OF-SLS-IN-INTRVAL}) is invoked. 	
\item If $h \geq L(I_j)$ then no further processing is required for $I_j$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\vspace{-0.8cm}
\item If $h < L(I_j)$. Then following steps are executed:
\begin{itemize}
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\item $I_j$ is deleted from $T[L(I_j)]$ and $I_j$ is inserted to $T[h]$. Set $h^{\prime}$ = $L(I_j)$ and $L(I_j)$ = $h$. 
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\item To recompute offset value for $I_j$ with new level value $h$, $\OFFSET$$(I_j)$ (Algorithm~\ref{alg:offset}) is invoked.  
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\item For every endpoint $t \in S$, it is checked if there is another interval at level $h^{\prime}$ that contains $t$. From property \textbf{P}, after changing level value of $I_j$ there can be at most two more intervals with level value $h^{\prime}$ that contains $t$. The check is done by performing an intersection query on $T[h^{\prime}]$ with $t$. If the query returns a NULL then $h^{\prime}$ is deleted from ${NZ}_t$ and $h^{\prime}$ is inserted to $Z_t$.\\  
	\end{itemize}
\end{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item[\textbf{Data structures and procedures used in insertion algorithm: }]
Let $I_i = [l_i, r_i]$ be the interval inserted in the $i$-th update step. We use $\Insertion$ (Algorithm~\ref{alg:insert}) to compute the color $(L(I_i),o(I_i))$ for interval $I_i$. Algorithm $\Insertion$ involves the following steps:
\begin{itemize}
\item \textbf{Computing $L(I_i)$: }\\
\textbf{Step 1: } Interval $I_i = [l_i, r_i]$ is inserted into $\mathcal{I}$. An intersection query is performed on $\mathcal{E}$ to check the presence of  
${I_{i}}^{l} = [l_i, l_i]$. If ${I_{i}}^{l}$ is in $\mathcal{E}$ then the algorithm proceeds to Step 2. Otherwise, procedure $\getSLS$($\mathcal{I},l_i$) (Algorithm~\ref{alg:GET-SLS}) is invoked. Procedure $\getSLS$($\mathcal{I},l_i$) works as follows: \\ 
an intersection query is performed on $\mathcal{I}$ with $I_i^{l}$. The query returns all the intervals in $\mathcal{I}$ which contain $I_i^{l}$. Let $\mathcal{I}_{I_i^{l}}$ denote the set returned by the intersection query. Red-Black trees $Z_{l_i}$ and ${NZ}_{l_i}$, each of size $\max(levels(\mathcal{I}_{I_i^{l}}))$, are created. For every $i$ in the range $[0,\max(levels(\mathcal{I}_{I_i^{l}}))]$, 
if $i \in levels(\mathcal{I}_{I_i^{l}})$ then $i$ is inserted to $Z_{l_i}$. Otherwise, $i$ is inserted to ${NZ}_{l_i}$. Same processing is repeated for $I_i^{r}$ = $[r_i,r_i]$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Step 2: } Procedure $\computemaxheightSLS$$(\mathcal{E},I_i)$ (Algorithm~\ref{alg:MAX-HEIGHT-OF-SLS-IN-INTRVAL}) is invoked to perform this step. The procedure works as follows:\\ 
to get the set of endpoints $S$ contained in interval $I_i$=$[l_i,r_i]$,  
an intersection query of $I_i$ is performed on $\mathcal{E}$. For every $t \in S$, $h_t$ is computed as follows:  if $Z_t$ is non-empty then the minimum value in $Z_t$ is assigned to $h_t$. Otherwise, $h_t$ is assigned a value one more than the maximum value in ${NZ}_t$. For every $t \in S$, the maximum value $h = \max\{h_t | t \in S\}$ is computed and level value of $I_i$, $L(I_i)$ is set to $h$.\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Step 3: }Procedure $\updateEndPoints$$(S,L(I_i))$ (Algorithm~\ref{algo:UPDATE-EDGE-POINTS}) is invoked to perform this step. The procedure works as follows:
for every $ t \in S$, $L(I_i)$ is deleted from $Z_t$ and inserted to ${NZ}_t$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item \textbf{Computing $o(I_i)$: } 
We use procedure $\OFFSET$$(I_i)$(Algorithm~\ref{alg:offset}) to compute $o(I_i)$. 
\end{itemize}
\end{description}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Analysis of $\Deletion$ and $\Insertion$ algorithm}
\label{subsec:analysis-fully-dynamic-algorithm}
In this section we present a worst case analysis of $\Deletion$ (Algorithm~\ref{alg:delete}) and $\Insertion$ (Algorithm~\ref{alg:insert}).
We analyze worst case performance of every step in  Algorithm~\ref{alg:delete} and present a worst case update time for deletion. Similarly, we analyze worst case performance of every step in $\Insertion$ and present a worst case update time for insertion. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Analysis of $\Deletion$ in the fully dynamic setting}
\label{subsubsec: analysis-fully-dynamic-deletion}
Let $I_i = [l_i,r_i]$ with color $(L(I_i), o(I_i))$  
be the interval presented to $\Deletion$ for deletion in the current update step. Let $n$ be the total number of intervals inserted during the course of execution of the algorithm. We present a worst case analysis of $\Deletion$ by analyzing the time required in every step of the algorithm. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{lem: deletion-step1}	
Step 1 of $\Deletion$ takes $O(\log n)$ time.
\end{lemma}
\begin{proof}
In Step $1$, interval $I_i$ is removed from interval tree $\mathcal{I}$ and interval tree $T[L(I_i)]$. Since $|\mathcal{I}| \leq n$ and $|T[L(I_i)]| \leq n$, this step takes $O(\log n)$
time in the worst case. Hence the Lemma.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{lem: deletion-step2}	
Step 2 of $\Deletion$ takes $O(\log n + \Delta)$ time.
\end{lemma}
\begin{proof}
In Step 2, to compute $\mathcal{E}_i$ = $\mathcal{E} \cap I_i$, an intersection query is performed on $\mathcal{E}$ with $I_i$. The time taken by the query to return the set $\mathcal{E}_i$ is $O(\log |\mathcal{E}| + |\mathcal{E}_i|)$. Since $|\mathcal{E}| \leq 2n$ and $|\mathcal{E}_i| \leq \Delta$, this step takes $O(\log n + \Delta)$ time in the worst case. Hence the Lemma.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{lem: deletion-step3}	
Step 3 of $\Deletion$ takes $O(\Delta \log n)$ time.
\end{lemma}
\begin{proof}
In Step 3, for every endpoint $t \in \mathcal{E}_i$, SLS $e_t$ is updated. To do so, it is checked if there is another interval with level value equal to $L(I_i)$ that contains $t$ using an intersection query on $T[L(I_i)]$ with $t$. Worst case time required by this query is $O(\log n + 2)$ = $O(\log n)$. If the intersection query returns NULL, then $L(I_i)$ is deleted from the tree ${NZ}_t$ and $L(I_i)$ is inserted to the tree $Z_t$. Since $|Z_t| \leq \omega$ and $|{NZ}_t| \leq \omega$, time required for deletion from ${NZ}_t$ and insertion to ${Z}_t$ is $O(\log \omega)$. Otherwise, if the intersection query returns a non-NULL value then no modifications are required for trees $Z_t$ and ${NZ}_t$. Therefore, total time required for one $t \in \mathcal{E}_i$ is $O(\log n + \log \omega)$. Since $|\mathcal{E}_i| \leq \Delta$, worst case time required by this step is $O(\Delta \log n + \Delta \log \omega)$ = $O(\Delta \log n)$. Hence the Lemma.
\end{proof}	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{lem: deletion-step4}	
Step 4 of $\Deletion$ takes $O(\Delta^2 \log n)$ time.
\end{lemma}
\begin{proof}
For the purpose of analysis, we visualize Step 4 in two phases where {\bf phase 1} comprises of computing the set $\D$ and {\bf phase 2} comprises of processing the set $\D$.\\	
{\bf phase 1: }In phase 1, set $\D$ = $\{I_j | L(I_j) > L(I_i), I_i \cap I_j \neq \phi \}$ is computed by using an intersection query on $\mathcal{I}$ with $I_i$. Let $H$ be the set returned by this query. Clearly $\D \subseteq H$, $|H| \leq \Delta$ and $|\mathcal{I}| \leq n$. Therefore, worst case time required by this query is $O(\log n + \Delta)$. Set $H$ is scanned and all the intervals whose level value is at most $L(I_i)$ are discarded in $O(\Delta)$ time. The remaining intervals are sorted in the increasing order of their level value and ties are broken in the increasing order of insertion time. Sorting all the remaining intervals takes $O(\Delta \log \Delta)$ time. %Insertion time is used to break the ties. 
Finally, the sorted set of intervals is the required set $\D$, where $|\D| \leq |H| \leq \Delta$. Therefore, phase 1 takes $O(\log n + \Delta \log \Delta)$ time.\\
{\bf phase 2: } 
In phase 2, every interval $I_j$ in the set $\D$ is processed as follows:
\begin{itemize}
	\item Procedure $\computemaxheightSLS$ is used to compute the set $S$ of supporting line segments contained in $I_j$ and maximum height $h$ any SLS contained in $S$. From Lemma~\ref{lem:runtimeComputemaxheightfullydynamic}, this step takes $O(\log n + \Delta \log \omega)$ time in the worst case.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item If $h \geq L(I_j)$ then no further processing is required for $I_j$. 
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item If $h < L(I_j)$. The following computation is done:
\begin{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item Deleting $I_j$ from $T[L(I_j)]$ and inserting $I_j$ into $T[h]$ takes $O(\log n)$ time. 
Let $h^{\prime}$ = $L(I_j)$. $L(I_j)$ is set to $h$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item To compute offset value of $I_j$ with new level value $h$, procedure $\OFFSET$$(I_j)$ is invoked. From Lemma~\ref{lem:time-greeyd-coloring}, procedure $\OFFSET$ takes $O(\log n)$ time in the worst case.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item For every endpoint $t \in S$, it is checked if there is another interval with level value $h^{\prime}$ that contains $t$. From property \textbf{P}, after changing level value of $I_j$ there can be at most two more intervals with level value $h^{\prime}$ that contains $t$.
It is checked by performing an intersection query on $T[h^{\prime}]$ with $t$. This query takes $O(\log n + 2)$ = $O(\log n)$ time in the worst case. If the intersection query returns NULL then $h^{\prime}$ is deleted from ${NZ}_t$ and $h^{\prime}$ is inserted to $Z_t$. Otherwise, if the intersection query returns a non-NULL value then no modifications are required for trees ${Z_t}$ and ${NZ}_t$. Time taken to perform all these operations for one SLS $e_t$ is $O(\log n + \log \omega)$. Therefore, worst case time taken for the entire set $S$ is $O(\Delta \log n + \Delta \log \omega)$ = $O(\Delta \log n)$. 
\end{itemize}
Therefore, the time taken for one interval $I_j \in \D$ is $O(\log n + \Delta)$ + $O(\Delta \log \omega)$ +$O(\Delta)$ +$O(\Delta \log n)$. For interval graphs, $\omega = \chi \leq \Delta+1$ and $\Delta + 1 \leq n$. Hence, time taken for one interval $I_j \in \D$ is $O(\Delta \log n)$. Since $|\D| \leq \Delta$, the time taken in phase 2 is $O(\Delta^{2} \log n)$. 
\end{itemize}
Therefore, total time taken by Step 4 of $\Deletion$ is the sum total of the time required in {\bf phase 1} and {\bf phase 2}, that is
$O(\log n+ \Delta \log \Delta)$ + $O(\Delta^{2}  \log n)$ = $O(\Delta^{2}  \log n)$ time. Hence the Lemma.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The update time of $\Deletion$ (Algorithm~\ref{alg:delete}) is given by the following theorem.
\begin{theorem}
\label{thm : fully-dynamic-update-time-deletion}
In the fully dynamic setting, deletion of an interval takes  $O(\Delta^{2} \log n)$ time in the worst case.
\end{theorem}
\begin{proof}
$\Deletion$ involves four steps. Lemma~\ref{lem: deletion-step1}, Lemma~\ref{lem: deletion-step2}, Lemma~\ref{lem: deletion-step3}, and Lemma~\ref{lem: deletion-step4} present the worst case time taken by every step. Therefore, we conclude that the worst case time $T$ taken by $\Deletion$ is: \\
$T$ = Worst Case Time for Step 1 + Worst Case Time for Step 2 + Worst Case Time for Step 3 + Worst Case Time for Step 4\\
$T$ = $O(\log n)$ + $O(\log n + \Delta)$ + $O(\Delta \log n)$ + $O(\Delta^{2} \log n)$\\
$T$ = $O(\Delta^{2} \log n)$
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Analysis of $\Insertion$ in fully dynamic setting}
\label{subsubsec: analysis-fully-dynamic-insertion}
Let $I_i$ = $[l_i,r_i]$ be the interval inserted in the $i$-th update step. We follow the same analysis as described in Section~\ref{subsection : Incremental-Algorithm-Analysis}. Running time of $\Insertion$(Algorithm~\ref{alg:insert}) in the fully dynamic setting differs from incremental setting because of the use of Red-Black trees to maintain supporting line segments instead of dynamic arrays and linked list.
\begin{itemize}
\item \textbf{Analysis of computing $L(I_i)$} :
\begin{lemma}
\label{lem: Fullydynamic-insertion-step1-analysis}	
Step $1$ in computing $L(I_i)$ of $\Insertion$ takes $O(\log n + \omega \log \omega)$ time. 	
\end{lemma}
\begin{proof}
Insertion of $I_i$ into $\mathcal{I}$ takes $O(\log n)$ time. Then procedure $\getSLS$ is invoked at both the endpoints of interval $I_i$. From Lemma~\ref{lem:runtimeComputeSLSfullyDynamic}, $\getSLS$ takes $O(\log n + \omega \log \omega)$. 	
Therefore, worst case time taken by Step 1 is $O(\log n + \omega \log \omega)$. Hence the Lemma.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{lem: Fullydynamic-insertion-step2-analysis}	
Step $2$ in computing $L(I_i)$ of $\Insertion$ takes $O(\log n + \Delta \log \omega)$ time. 	
\end{lemma}
\begin{proof}
Procedure $\computemaxheightSLS$(Algorithm~\ref{alg:MAX-HEIGHT-OF-SLS-IN-INTRVAL}) is invoked for this step. From Lemma~\ref{lem:runtimeComputemaxheightfullydynamic}, $\computemaxheightSLS$ takes $O(\log n + \Delta \log \omega)$ time. Hence the Lemma.  
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{lem: Fullydynamic-insertion-step3-analysis}	
Step $3$ in computing $L(I_i)$ of $\Insertion$ takes $O(\Delta \log \omega)$ time. 	
\end{lemma}
\begin{proof}
Procedure $\updateEndPoints$ (Algorithm~\ref{algo:UPDATE-EDGE-POINTS}) is invoked for this step. From Lemma~\ref{lem:runtimeUpdaeSLSfullydynamic}, $\updateEndPoints$ takes $O(\Delta \log \omega)$ time. Hence the Lemma.   
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item \textbf{Analysis of computing $o(I_i)$} :
\begin{lemma}
\label{lem:time-greeyd-coloring-fullydynamic}
In $\Insertion$, computing the offset value of the interval $I_i$ with level value $L(I_i)$ takes $O(\log n)$ time in the worst case.
\end{lemma}
\begin{proof}
Proof is same as the proof of Lemma~\ref{lem:time-greeyd-coloring}.
\end{proof}
\end{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The update time of $\Insertion$(Algorithm~\ref{alg:insert}) is given by the following theorem.
\begin{theorem}
\label{thm :fully-dynamic-update-time-insertion}
In the fully dynamic setting, insertion of an interval takes  $O(\log n + \Delta \log \omega)$ time in the worst case.
\end{theorem}
\begin{proof}
Our insertion algorithm involves two phases : computing level value and computing offset value. Computing level value involves $3$ steps. In Lemma~\ref{lem: Fullydynamic-insertion-step1-analysis}, Lemma~\ref{lem: Fullydynamic-insertion-step2-analysis}, and Lemma~\ref{lem: Fullydynamic-insertion-step3-analysis} we present the worst case time taken by each of these steps. In Lemma~\ref{lem:time-greeyd-coloring-fullydynamic} we present the worst case time taken in computing offset value. Therefore, we conclude that the worst case time $T$ taken by our insertion algorithm is :\\
$T$ = Worst case time taken to compute the level value + Worst case time taken to compute the offset value \\
$T$ = Worst case time taken by Step 1 + Worst case time taken by Step 2 + Worst case time taken by Step 3 + Worst case time taken to compute the offset value \\
$T$ = $O(\log n + \omega \log \omega)$ + $O(\log n + \Delta \log \omega)$ + $O(\Delta \log \omega)$ + $O(\log n)$ \\
$T$ = $O(\log n + \Delta \log \omega)$ 
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Combining Theorem~\ref{thm : fully-dynamic-update-time-deletion} and Theorem~\ref{thm :fully-dynamic-update-time-insertion} we present our fully dynamic result in the following theorem.
\begin{theorem}
\label{thm : update-time-fully-dynamic}
There exists a fully dynamic algorithm which supports insertion of an interval in  $O(\log n + \Delta \log \omega)$ and deletion of an interval in  $O(\Delta^{2} \log n)$ worst case time. 
\end{theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\noindent


==> Journal/Incremental_copy.tex <==
% !TEX root = ../IntervalColoringFullVersion.tex
\section{Incremental Algorithm using supporting line segment}
\label{sec: Incremental-Algorithm}
In the incremental setting, for each $1 \leq i \leq n$, $I_i = [l_i,r_i]$ represents the interval inserted in the $i$-th update step. Here $n$ is the total number of insertions. In this section, we design an incremental algorithm ($\Insertion$) for proper interval coloring which is an implementation of $\KTSLS$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Algorithm $\Insertion$}
\label{subsec:incrementalAlgo}
We present the pseudo code of $\Insertion$ in Algorithm~\ref{alg:insert} and a summarized description of the procedures used in $\Insertion$ in Table~\ref{table:2}. Algorithm $\Insertion$ computes the color $(L(I_i),o(I_i))$ by implementing the steps as described below:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{enumerate}
	\item {\bf Computing $L(I_i)$:}\\
	\textbf{Step 1}: Insert $I_i$ into the set of intervals $\mathcal{I}$ (Line 1 in Algorithm~\ref{alg:insert}). Check if the endpoint $l_i$ is already present in set of endpoints $\mathcal{E}$ (Line 4 in Algorithm~\ref{alg:insert}). If not then compute the SLS at endpoint $l_i$ (Line 5 in Algorithm~\ref{alg:insert}) and insert $l_i$ into the set $\mathcal{E}$ (Line 6 in Algorithm~\ref{alg:insert}). Repeat the same processing for endpoint $r_i$ (Line 8-11 in Algorithm~\ref{alg:insert}).\\
	\textbf{Step 2}: Compute the set $S = \mathcal{E} \cap I_i$.  For each $t \in S$, compute $h_t$, the height of the SLS $e_t$ at $t$.  
	Assign $L(v_i) = \displaystyle \max_{t \in S} h_t$ (Line 12-13 in Algorithm~\ref{alg:insert}).\\
	\textbf{Step 3}: Update the SLS $e_t$ for each point $t \in S$ (Line 14 in Algorithm~\ref{alg:insert}). 
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\item {\bf Computing $o(I_i)$}:
	Compute $o(I_i)$ to be the smallest value from the set $\{1,2,3\}$ that is different from the offset values of the neighbours of $I_i$ which have the level $L(I_i)$ (Line 15 in Algorithm~\ref{alg:insert}). 
\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We present description of the procedures used in $\Insertion$ in Section~\ref{subssec:procedures-handle-insert}.
% We analyze update time of $\Insertion$ in Section~\ref{subsection : Incremental-Algorithm-Analysis}.  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[h]	
	\caption{$\Insertion$($I_i = [l_i,r_i]$) is used to handle insertion of interval $I_i$}
	\begin{algorithmic}[1]
		\State $\mathcal{I}$.insert($I_i$) 
		\State $I_i^{l} \gets$ $[l_i,l_i]$   
		\State $I_i^{r} \gets$ $[r_i,r_i]$   
		\If{($\mid \mathcal{E}$.intersection($I_i^{l}) \mid$ = $0$)} 
		\State $A_{l_i}, Q_{l_i} \leftarrow$  \Call{$\getSLS$}{$\mathcal{I}$,$l_i$} 
		\State $\mathcal{E}$.insert($I_i^{l}$) 
		\EndIf
		\If{($\mid \mathcal{E}$.intersection($I_i^{r}) \mid$ = $0$)}  
		\State $A_{r_i}, Q_{r_i} \leftarrow$  \Call{$\getSLS$}{$\mathcal{I}$,$r_i$} 
		\State $\mathcal{E}$.insert($I_i^{r}$) 
		\EndIf
		\State $S, h \leftarrow$  \Call{$\computemaxheightSLS$}{$\mathcal{E}$,$I_i$}
		\State $L(I_i) \leftarrow h$
		\State \Call{$\updateEndPoints$}{$S,L(I_i)$}
		\State \Call{$\OFFSET$}{$I_i$}
	\end{algorithmic}
	\label{alg:insert}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
	\centering
	\begin{tabular}{|l|l|l|} 
		\hline
		\multicolumn{3}{|l|}{$\getSLS$$(\mathcal{I},t)$}\\
		\hline
		Description & Worst-case  & Return\\
		& Running Time & Value \\
		\hline
		Computes the supporting line segment for endpoint $t$ & $O(\log(n)+\omega)$ & $A_t, Q_t$\\
		and maintains it using dynamic array $A_t$ and doubly linked list $Q_t$.  & (Lemma~\ref{lem:runningtime-computeSLS}) & \\
		\hline
		\hline
		\multicolumn{3}{|l|}{$\computemaxheightSLS$$(\mathcal{E},I_i)$}\\
		\hline
		Description & Worst-case  & Return\\
		& Running Time & Value \\
		\hline
		From the interval tree $\mathcal{E}$, computes the set of endpoints $S$   & $O(\log(n)+\Delta)$ & $S,h$\\
		contained in the interval $I_i$ and for each $t \in S$, & (Lemma~\ref{lem:runningTimeMaxHeightofSLS}) & \\
		from the doubly linked list $Q_t$ computes the  height $h_t$  & & \\
		and returns $h$ = $\max\{h_t | t \in S\}$ & & \\
		\hline
		\hline
		\multicolumn{3}{|l|}{$\updateEndPoints$$(S,L(I_i))$}\\
		\hline
		Description & Amortized  & Return \\
		& Running Time & Value \\
		\hline
		Updates the endpoints in $S$ to reflect the addition of a new interval & $O(\Delta)$ & - \\
		interval $I_i$ at level $L(I_i)$.
		This updates the  dynamic array $A_t$ & (Lemma~\ref{lem:runningTimeUpdateEndpoints}) & \\
		and the doubly linked list $Q_t$ for each $t \in S$  & & \\
		\hline
		\hline
		\multicolumn{3}{|l|}{$\OFFSET$$(I_i)$}\\
		\hline
		Description & Worst-case & Return\\
		& Running Time & Value \\
		\hline
		Assigns an offset value to $I_i$ from $\{1,2,3\}$ & $O(\log(n))$ & -\\
		by considering the offset of the intervals  & (Lemma~\ref{lem:time-greeyd-coloring}) & \\
		intersecting it in $T[L(I_i)]$ where $L(I_i)$ is the level value of $I_i$ & & \\
		\hline
	\end{tabular}
	\caption{Procedures used in $\Insertion$ (Algorithm~\ref{alg:insert}) }
	\label{table:2}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The amortized update time of $\Insertion$ is given by the Theorem~\ref{thm:IncrementalAlgo}. 
\begin{theorem}
	\label{thm:IncrementalAlgo}
	There exists an incremental algorithm which supports insertion of 	
	a sequence of $n$ intervals in amortized $O(\log n + \Delta)$ time per update.
\end{theorem}
\begin{proof}
	We analyze $\Insertion$ by analyzing the time required in every step of the algorithm. 
	\begin{enumerate}
		\item \textbf{Analysis for computing $L(I_i)$:}\\
		Computing $L(I_i)$ involves $3$ steps.
		\begin{enumerate}
			\item Step 1 in computing $L(I_i)$ for interval $I_i$ takes $O(\log n + \omega)$ time: Insertion of $I_i$ = $[l_i,r_i]$ into $\mathcal{I}$ takes $O(\log n)$ time. Let $I_i^{l}$ = $[l_i,l_i]$. Checking if $I_i^{l}$ is present in $\mathcal{E}$ by an intersection query takes $O(\log n)$ time in the worst case. 
			\begin{itemize}
				\item If $I_i^{l}$ is in $\mathcal{E}$. Then no further processing is done in Step 1.
				\item If $I_i^{l}$ is not in $\mathcal{E}$ then procedure $\getSLS$($\mathcal{I},l_i$) is invoked.
				From Lemma~\ref{lem:runningtime-computeSLS}, procedure $\getSLS$ takes $O(\log n + \omega)$ time.    
			\end{itemize}
			Same processing is repeated for $I_i^{r}$ = $[r_i,r_i]$. Hence Step 1 in computing $L(I_i)$ for interval $I_i$ takes $O(\log n + \omega)$ time.
			%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
			\item Step 2 in computing $L(I_i)$ for interval $I_i$ takes $O(\log n + \Delta)$ time: Procedure $\computemaxheightSLS$$(\mathcal{E},I_i)$ is invoked to perform this step. From Lemma~\ref{lem:runningTimeMaxHeightofSLS}, procedure $\computemaxheightSLS$(Algorithm~\ref{alg:MAX-HEIGHT-OF-SLS-IN-INTRVAL-usingDynamicArray}) takes $O(\log n + \Delta)$ time. Hence Step 2 in computing $L(I_i)$ for interval $I_i$ takes $O(\log n + \Delta)$ time. 
			%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
			\item Step $3$ in computing $L(I_i)$ for interval $I_i$ takes amortized $O(\Delta)$ time: Procedure $\updateEndPoints$$(S,L(v_i))$ is invoked to perform this step. From Lemma~\ref{lem:runningTimeUpdateEndpoints}, procedure $\updateEndPoints$(Algorithm~\ref{algo:UPDATE-EDGE-POINTS-usingDynamicArray}) takes amortized $O(\Delta)$ time. Hence Step $3$ in computing $L(I_i)$ for interval $I_i$ takes amortized $O(\Delta)$ time. 
		\end{enumerate}
		\item \textbf{Analysis for computing $o(I_i)$:}\\ 
		To compute the offset value of interval $I_i$ with level value $L(I_i)$, procedure $\OFFSET$$(I_i)$ is invoked. From Lemma~\ref{lem:time-greeyd-coloring}, procedure $\OFFSET$$(I_i)$ takes $O(\log n)$ time.
	\end{enumerate}	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%	
	For interval graphs, it is well known that $\omega=\chi \leq\Delta+1$. Therefore, total time taken by $\Insertion$ for insertion of $n$ intervals is:\\
	$\mathcal{T}$ = Total time for Step1 + Total Time for Step 2 + Total Time for Step 3 + Total time for computing offset \\
	$\mathcal{T}$ = $n \times O(\log n + \omega)$ + $n \times O(\log n + \Delta)$ + $n \times O(\Delta)$ + $n \times O(\log n)$\\
	$\mathcal{T}$ = $O(n\log n + n \Delta)$\\
	Therefore, the amortized update time over a sequence of $n$ interval insertions is  $O(\log n + \Delta)$. 
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Procedures used in $\Insertion$}
\label{subssec:procedures-handle-insert}
\noindent
We present a description of the different procedures used in $\Insertion$ below.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\noindent\begin{minipage}{\textwidth}
 %  \centering
 \noindent
   \begin{minipage}{.45\textwidth}
   \begin{algorithm}[H]
  \caption{ $\getSLS$($\mathcal{I}$,$t$) is used to compute the supporting line segment at endpoint $t$. In this procedure SLS is maintained using dynamic array and doubly linked list.}
	\begin{algorithmic}[1]
		\Procedure{$\getSLS$}{$\mathcal{I}$,$t$}
		\State $\mathcal{I}_t \leftarrow \mathcal{I}$.intersection($[t,t]$)
		\State $h_t, U \leftarrow 0, \{\}$
		\State $A_t \leftarrow [\ ]$
		\State $Q_t \leftarrow $ Empty doubly linked list
		\For{$I$ \textbf{in} $\mathcal{I}_t$}
		\State $h_t \leftarrow \max(h_t,L(I))$
		\State $U$.insert$(L(I))$
		\EndFor
		\For{$i$ \textbf{in} $\{0,1,2,...h_t\}$} 
		\State $A_t$.at$(i) \leftarrow $  0
		\State $Q_t$.insert$(i)$
		\EndFor
		\For{$i$ \textbf{in} $U$.begin() \textbf{to} $U$.end()} 
		\State $A_t.$at$(i) \leftarrow$  1
		\State $Q_t$.delete$(i)$
		\EndFor
		\State \Return $A_t, Q_t$
		\EndProcedure
	\end{algorithmic}
	\label{alg:GET-SLS-dynamicArray}
	\end{algorithm}
	\end{minipage}
	\hspace{.6cm}
	%\vspace{-3cm}
   \begin{minipage}{.45\textwidth}
%\centering
     \begin{algorithm}[H]
     \caption{$\computemaxheightSLS$($\mathcal{E}$,$I$) is used to compute the set $S$ of endpoints contained in interval $I$ and compute the maximum height $h$ of all the supporting line segments at these endpoints. In this procedure SLS is maintained using dynamic array and doubly linked list.}
	\begin{algorithmic}[1]
		\Procedure{$\computemaxheightSLS$}{$\mathcal{E}$,$I$} 
		\State $S \leftarrow  \mathcal{E}$.intersection($I$)
		\State $h \leftarrow 0$
		\For{$t$ \textbf{in} $S$}
		\If{$Q_t$.begin() is NULL}
		\State $h_t \leftarrow $0
		\Else 
		\State $h_t \leftarrow {Q_t}$.begin() 
		\EndIf
		\State $h \leftarrow \max(h,h_t)$
		\EndFor
		\State return $S, h$
		\EndProcedure
	\end{algorithmic}
	\label{alg:MAX-HEIGHT-OF-SLS-IN-INTRVAL-usingDynamicArray}
	\end{algorithm}
   \end{minipage}
   
   \noindent
      \begin{minipage}{.45\textwidth}
   \begin{algorithm}[H]
	\caption{$\updateEndPoints$($S$,$L(I)$) is used to update the supporting line segments at the endpoints contained in set $S$ for level value $L(I)$. In this procedure SLS is maintained using dynamic array and doubly linked list.}
	\begin{algorithmic}[1]
		\Procedure{$\updateEndPoints$}{$S$,$L(I)$}
		\State $l \leftarrow L(I)$ 
		\For{$t$ \textbf{in} $S$}
		\If{$l > A_t$.size()}
		\For{$i$ \textbf{in} $\{A_t$.size()$+1, l\}$ }
		\State {$A_t$.at$(i) \leftarrow$ 0}
		\State $Q_t$.insert$(i)$
		\EndFor
		\EndIf
		\State{$A_t$.at$(l) \leftarrow$  1}
		\State{$Q_t$.delete$(l)$}
		\State{$h_t \leftarrow Q_t$.begin()} 
		\EndFor
		\EndProcedure
	\end{algorithmic}
	\label{algo:UPDATE-EDGE-POINTS-usingDynamicArray}
\end{algorithm}
\end{minipage}
   \begin{minipage}{.45\textwidth}
\begin{algorithm}[H]
	\caption{$\OFFSET$($I$) is used to compute the offset value of the interval $I$ with level value $L(I)$. }
	\begin{algorithmic}[1]
		\Procedure{$\OFFSET$}{I}
		\If{$T[L(I)]$ \textbf{is} \textit{NULL}}
		\State $T[L(I)] \leftarrow $ \Call{Interval\_Tree}{\ }
		\EndIf
		\State S $ \leftarrow T[L(I)].$intersection($I$)
		\State $o(I) \leftarrow$  The minimum value in the set $\{1, 2, 3\}$ which is not the offset value of any interval in S. 
		\State $T[L(I)].$insert($I$)
		\EndProcedure
	\end{algorithmic}
	\label{alg:offset}
\end{algorithm}
\end{minipage}
 %  \captionof{figure}{Two algorithms side by side}
 %  \label{fig:twoalg}
%\end{minipage}
\begin{enumerate}
\item \textbf{Procedure $\getSLS$($\mathcal{I}_t, t$):} This procedure is used to compute the SLS at endpoint $t$. It works as follows (Algorithm~\ref{alg:GET-SLS-dynamicArray}): it performs an intersection query on $\mathcal{I}$ with interval $[t,t]$. Let $\mathcal{I}_t$ denotes the set returned by the intersection query. Dynamic arrays $A_{t}$ and $A^{\prime}_{t}$, each of size $\max(levels(\mathcal{I}_{t}))$, are created. For every $i$ in the range $[0, \max(levels(\mathcal{I}_{t}))]$, $A_t[i]$ is set to $1$ if $i \in levels(\mathcal{I}_t)$ and $A_t[i]$ is set to $0$ otherwise. For every $A_t[i]$ = $0$, a node storing the index $i$ is inserted to the doubly linked list $Q_t$ and pointer to that node is stored in $A^{\prime}_t[i]$. For every $A_t[i]$ = $1$, we store a NULL in $A^{\prime}_t[i]$.
\begin{algorithm}[H]
	\caption{ $\getSLS$($\mathcal{I}$,$t$) is used to compute the supporting line segment at endpoint $t$. In this procedure SLS is maintained using dynamic array and doubly linked list.}
	\begin{algorithmic}[1]
		\Procedure{$\getSLS$}{$\mathcal{I}$,$t$}
		\State $\mathcal{I}_t \leftarrow \mathcal{I}$.intersection($[t,t]$)
		\State $h_t, U \leftarrow 0, \{\}$
		\State $A_t \leftarrow [\ ]$
		\State $Q_t \leftarrow $ Empty doubly linked list
		\For{$I$ \textbf{in} $\mathcal{I}_t$}
		\State $h_t \leftarrow \max(h_t,L(I))$
		\State $U$.insert$(L(I))$
		\EndFor
		\For{$i$ \textbf{in} $\{0,1,2,...h_t\}$} 
		\State $A_t$.at$(i) \leftarrow $  0
		\State $Q_t$.insert$(i)$
		\EndFor
		\For{$i$ \textbf{in} $U$.begin() \textbf{to} $U$.end()} 
		\State $A_t.$at$(i) \leftarrow$  1
		\State $Q_t$.delete$(i)$
		\EndFor
		\State \Return $A_t, Q_t$
		\EndProcedure
	\end{algorithmic}
	\label{alg:GET-SLS-dynamicArray}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{lem:runningtime-computeSLS}
Procedure $\getSLS$ takes $O(\log n + \omega)$ time. 
\end{lemma}
\begin{proof}
Intersection query takes $O(\log|\mathcal{I}| + |\mathcal{I}_t|)$ time. Computing dynamic arrays $A_{t}$, $A^{\prime}_{t}$, and doubly linked list $Q_{t}$ takes $O(\max(levels(\mathcal{I}_{t})))$ time. Since $\max(levels(\mathcal{I}_{t})) \leq \omega$, time taken for the operations on dynamic arrays and associated linked list is $O(\omega)$. Total time taken by procedure $\getSLS$$(\mathcal{I},t)$ is $O(\log|\mathcal{I}| + |\mathcal{I}_{t}|)$ + $O(\omega)$ = $O(\log|\mathcal{I}| + |\mathcal{I}_{t}| + \omega)$. At any level, SLS ${e_t}$ intersects with at most $2$ intervals and we have $\omega$ many levels. Hence, $|\mathcal{I}_{t}|$ = $O(\omega)$. Again, $|\mathcal{I}| \leq n$. Therefore, time taken by procedure $\getSLS$ in the worst case is $O(\log n + \omega)$. Hence the Lemma.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item \textbf{Procedure $\computemaxheightSLS$$(\mathcal{E}, I_i)$:} This procedure is used to compute the maximum height of SLS contained in interval $I_i$. It works as follows (Algorithm~\ref{alg:MAX-HEIGHT-OF-SLS-IN-INTRVAL-usingDynamicArray}): it performs an intersection query of $I_i$ on $\mathcal{E}$. This query returns the set $S$ of all the endpoints that intersect with $I_i$. Let $h$ denote the maximum height of SLS at any endpoint $t \in S$. The procedure returns $h$ and the set $S$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[H]
	\caption{$\computemaxheightSLS$($\mathcal{E}$,$I$) is used to compute the set $S$ of endpoints contained in interval $I$ and compute the maximum height $h$ of all the supporting line segments at these endpoints. In this procedure SLS is maintained using dynamic array and doubly linked list.}
	\begin{algorithmic}[1]
		\Procedure{$\computemaxheightSLS$}{$\mathcal{E}$,$I$} 
		\State $S \leftarrow  \mathcal{E}$.intersection($I$)
		\State $h \leftarrow 0$
		\For{$t$ \textbf{in} $S$}
		\If{$Q_t$.begin() is NULL}
		\State $h_t \leftarrow $0
		\Else 
		\State $h_t \leftarrow {Q_t}$.begin() 
		\EndIf
		\State $h \leftarrow \max(h,h_t)$
		\EndFor
		\State return $S, h$
		\EndProcedure
	\end{algorithmic}
	\label{alg:MAX-HEIGHT-OF-SLS-IN-INTRVAL-usingDynamicArray}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{lem:runningTimeMaxHeightofSLS}
Procedure $\computemaxheightSLS$ takes $O(\log n + \Delta)$ time.
\end{lemma}
\begin{proof}
The intersection query takes time $O(\log |\mathcal{E}| + |S|)$. Finding the height of SLS at one endpoint takes constant time. Therefore, finding the maximum height of SLS at any endpoint contained in $S$ takes $O(|S|)$ time. Since $\Delta$ is the maximum degree in the associated interval graph, interval $I_i$ can intersect with at most $\Delta$ intervals. Therefore, $|S|$ = $O(\Delta)$. Again, $|\mathcal{E}| \leq 2n$. Thus the worst case time taken by $\computemaxheightSLS$ is $O(\log n + \Delta)$. Hence the Lemma.	
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item \textbf{Procedure $\updateEndPoints$$(S,L(I_i))$: } This procedure is used to update the SLS at the endpoints contained in set $S$. It works as follows (Algorithm~\ref{algo:UPDATE-EDGE-POINTS-usingDynamicArray}): let $l = L(I_i)$. For every endpoint $t \in S$, size of $A_t$ is checked.  
\begin{enumerate}
	\item 
	%\label{case:1}
	{\bf Case A:} If $l < {A_t}$.size(). In this case, $A_t[l]$ is set to $1$. The pointer stored in $A^{\prime}_t[l]$ is used to delete the node in $Q_t$ which stores the value $l$ and $A^{\prime}_t[l]$ is set to NULL subsequently. If the deleted node in $Q_t$ was the head node, then the head node is updated to the next node in $Q_t$ and thus the value of $h_t$ also gets updated.  
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\item 
	%\label{case :2}
	{\bf Case B:} If $l \geq {A_t}$.size(). In this case, the standard doubling technique for expansion of dynamic arrays \cite{Cormen:2009:IAT:1614191} is used to increase the size of $A_t$ until ${A_t}$.size() becomes strictly greater than $l$.  $A^{\prime}_t$ is also expanded along with $A_t$ and appropriate nodes are inserted to $Q_t$. Once ${A_t}$.size() $> l$, the remaining operations are same as in the case \textbf{A}.   
\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[H]
	\caption{$\updateEndPoints$($S$,$L(I)$) is used to update the supporting line segments at the endpoints contained in set $S$ for level value $L(I)$. In this procedure SLS is maintained using dynamic array and doubly linked list.}
	\begin{algorithmic}[1]
		\Procedure{$\updateEndPoints$}{$S$,$L(I)$}
		\State $l \leftarrow L(I)$ 
		\For{$t$ \textbf{in} $S$}
		\If{$l > A_t$.size()}
		\For{$i$ \textbf{in} $\{A_t$.size()$+1, l\}$ }
		\State {$A_t$.at$(i) \leftarrow$ 0}
		\State $Q_t$.insert$(i)$
		\EndFor
		\EndIf
		\State{$A_t$.at$(l) \leftarrow$  1}
		\State{$Q_t$.delete$(l)$}
		\State{$h_t \leftarrow Q_t$.begin()} 
		\EndFor
		\EndProcedure
	\end{algorithmic}
	\label{algo:UPDATE-EDGE-POINTS-usingDynamicArray}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{lem:runningTimeUpdateEndpoints}
Procedure $\updateEndPoints$ takes $O(\Delta)$ amortized time.
\end{lemma}
\begin{proof}
For every endpoint $t \in S$, size of $A_t$ is checked in constant time. To analyze the time required in $\updateEndPoints$, we observe that every update must perform the operations as described in case \textbf{A}. We refer to these operations as \textit{task M}(M stands for mandatory). Some updates have to perform additional operations as described in case \textbf{B}. We refer to these operations as \textit{task A}(A stands for additional). 
The time taken by each update to perform \textit{task M} is $|S| \times O(1) = O(|S|)$. Since $\Delta$ is the maximum degree, it follows that $|S| \leq \Delta$. Therefore, every update takes $O(\Delta)$ time to perform \textit{task M} in the worst case. To analyze the time required to perform \textit{task A}, we crucially use the fact that our algorithm is incremental and hence only expansions of the dynamic arrays take place. Since $\omega$ is the size of the maximum clique, it follows that the maximum size of a dynamic array throughout the entire execution of the algorithm is upper bounded by $2\omega$. Over a sequence of $n$ insertions, the total number of endpoints is upper bounded by $2n$. Therefore, we maintain at most $4n$ dynamic arrays. For every such array,  total number of inserts in the array and the associated doubly linked list is at most $2 \omega$ in the entire run of the algorithm. An insertion into the dynamic array takes constant amortized time and insertion into doubly linked list takes constant worst case time. Therefore, during the entire run of the algorithm total time required to perform \textit{task A} on one dynamic array and its associated doubly linked list is $O(\omega)$. This implies that during the entire run of the algorithm total time spent on \textit{task A} over all the updates is $\leq 4n \times O(\omega)$. Let ${\sf T}$ be the total time spent on $\updateEndPoints$ at the end of $n$ insertions. This is the sum of the total time for \textit{task A} and the total time for \textit{task M}. Therefore, \\
${\sf T} \leq 4n \times O(\omega) + n \times O(\Delta)$\\
${\sf T} \leq 4n \times O(\Delta) + n \times O(\Delta)$ [since $\omega \leq \Delta + 1$]\\
Therefore, ${\sf T} = O(n \Delta)$. Hence the Lemma.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item \textbf{Procedure $\OFFSET$$(I_i)$: } This procedure is used to compute the offset value of interval $I_i$ with level value $L(I_i)$. 
\begin{algorithm}[H]
	\caption{$\OFFSET$($I$) is used to compute the offset value of the interval $I$ with level value $L(I)$. }
	\begin{algorithmic}[1]
		\Procedure{$\OFFSET$}{I}
		\If{$T[L(I)]$ \textbf{is} \textit{NULL}}
		\State $T[L(I)] \leftarrow $ \Call{Interval\_Tree}{\ }
		\EndIf
		\State S $ \leftarrow T[L(I)].$intersection($I$)
		\State $o(I) \leftarrow$  The minimum value in the set $\{1, 2, 3\}$ which is not the offset value of any interval in S. 
		\State $T[L(I)].$insert($I$)
		\EndProcedure
	\end{algorithmic}
	\label{alg:offset}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The procedure $\OFFSET$(Algorithm~\ref{alg:offset}) works as follows: hash table $T$ is used to access the interval tree $T[L(I_i)]$. If $T[L(I_i)]$ is NULL, then an interval tree $T[L(I_i)]$ is created with $I_i$ as the first interval. Otherwise, $T[L(I_i)]$ is the interval tree which stores all the intervals with level value same as $L(I_i)$. An intersection query is performed on $T[L(I_i)]$ with $I_i$ to obtain all the intervals that intersect with $I_i$. From Property {\bf P}, the maximum intervals returned by the above query is $2$. The offset value of interval $I_i$, $o(I_i)$, is set to be the smallest value from $\{1,2,3\}$ not assigned to any of the at most two neighbors of $I_i$ in level $L(I_i)$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{lem:time-greeyd-coloring}	
Procedure $\OFFSET$ takes $O(\log n)$ time.
\end{lemma}
\begin{proof}
Hash table $T$ is used to access the interval tree $T[L(I_i)]$ in constant time. If $T[L(I_i)]$ is NULL, then an interval tree $T[L(I_i)]$ is created with $I_i$ as the first interval in constant time. Otherwise, $T[L(I_i)]$ is the interval tree which stores all the intervals with level value same as $L(I_i)$. Intersection query on $T[L(I_i)]$ with $I_i$ takes $O(\log |\mathcal{I}| + 2)$ = $O(\log n +2)$ = $O(\log n)$ time. The offset value for interval $I_i$, $o(I_i)$, is selected from $\{1,2,3\}$ in constant time. Hence the Lemma.
\end{proof}
\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\subsection{Analysis of $\Insertion$}
\label{subsection : Incremental-Algorithm-Analysis}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section we analyze $\Insertion$ by analyzing the time required in every step of the algorithm.
\begin{enumerate}
\item \textbf{Analysis for computing $L(I_i)$:}\\
Computing $L(I_i)$ involves $3$ steps (see Section~\ref{subsec:incrementalAlgo}).\\  
\begin{lemma}
\label{lem:step1-time}
Step 1 in computing $L(I_i)$ for interval $I_i$ takes $O(\log n + \omega)$ time.
\end{lemma}
\begin{proof} 
Insertion of $I_i$ = $[l_i,r_i]$ into $\mathcal{I}$ takes $O(\log n)$ time. Let $I_i^{l}$ = $[l_i,l_i]$. Checking if $I_i^{l}$ is present in $\mathcal{E}$ by an intersection query takes $O(\log n)$ time in the worst case. 
\begin{itemize}
	\item If $I_i^{l}$ is in $\mathcal{E}$. Then no further processing is done in Step 1.
	\item If $I_i^{l}$ is not in $\mathcal{E}$ then procedure $\getSLS$($\mathcal{I},l_i$) is invoked.
	From Lemma~\ref{lem:runningtime-computeSLS}, procedure $\getSLS$ takes $O(\log n + \omega)$ time.    
\end{itemize}
Same processing is repeated for $I_i^{r}$ = $[r_i,r_i]$. Hence the Lemma.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{lem:step2-time}
Step 2 in computing $L(I_i)$ for interval $I_i$ takes $O(\log n + \Delta)$ time.
\end{lemma}
\begin{proof}
Procedure $\computemaxheightSLS$$(\mathcal{E},I_i)$ is invoked to perform this step. From Lemma~\ref{lem:runningTimeMaxHeightofSLS}, procedure $\computemaxheightSLS$(Algorithm~\ref{alg:MAX-HEIGHT-OF-SLS-IN-INTRVAL-usingDynamicArray}) takes $O(\log n + \Delta)$ time. Hence the Lemma.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{lem:step3-time}
Step $3$ in computing $L(I_i)$ for interval $I_i$ takes amortized $O(\Delta)$ time.
\end{lemma}
\begin{proof}
Procedure $\updateEndPoints$$(S,L(v_i))$ is invoked to perform this step. From Lemma~\ref{lem:runningTimeUpdateEndpoints}, procedure $\updateEndPoints$(Algorithm~\ref{algo:UPDATE-EDGE-POINTS-usingDynamicArray}) takes amortized $O(\Delta)$ time. Hence the Lemma.	
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item \textbf{Analysis for computing $o(I_i)$:}\\ 
To compute the offset value of interval $I_i$ with level value $L(I_i)$, procedure $\OFFSET$$(I_i)$ is invoked. From Lemma~\ref{lem:time-greeyd-coloring}, procedure $\OFFSET$$(I_i)$ takes $O(\log n)$ time. 	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{enumerate} 
\end{comment}
